Evolution of states and mesoscopic scaling for two-component birth-and-death dynamics in continuum

Two coupled spatial birth-and-death Markov evolutions on $\mathbb{R}^d$ are obtained as unique weak solutions to the associated Fokker-Planck equations. Such solutions are constructed by its associated sequence of correlation functions satisfying the so-called Ruelle-bound. Using the general scheme of Vlasov scaling we are able to derive a system of non-linear, non-local mesoscopic equations describing the effective density of the particle system. The results are applied to several models of ecology and biology.

==> jinfo.tex <==
\jvolume{22}
\jyear{2016}
\jnumber{4}

